Optimal Delegation in Markets for Matching with Signaling

This paper studies a delegation problem faced by the planner who wants to regulate receivers' reaction choices in markets for matching between receivers and senders with signaling. We provide a noble insight into the planner's willingness to delegate and the design of optimal (reaction) interval delegation as a solution to the planner's general mechanism design problem. The relative heterogeneity of receiver types and the productivity of the sender' signal are crucial in deriving optimal interval delegation in the presence of the trade-off between matching efficiency and signaling costs.

==> figures_tables/beta_qa_change_shape1_1_shape2_1_short.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Thu Feb 23 10:55:56 2023
\begin{table}[hp]
\centering
\caption{Design 4 with Beta(1,1)} 
\begingroup\footnotesize
\begin{tabular}{rrrrrrrrr}
  \hline
$q$ & $k$ & $a$ & $\bar{z}$ & $\bar{x}$ & $t_h$ & $z_h$ & $x_h$ & $s_h$ \\ 
  \hline
1.00 & 1.00 & 0.00 & 3.00 & 3.00 & 0.60 & 0.40 & 0.40 & 0.70 \\ 
  1.10 & 1.00 & 0.00 & 3.00 & 3.40 & 0.70 & 0.50 & 0.40 & 0.80 \\ 
  1.20 & 1.00 & 0.00 & 3.00 & 3.70 & 0.80 & 0.60 & 0.50 & 0.90 \\ 
  1.30 & 1.00 & 0.00 & 3.00 & 4.20 & 0.90 & 0.70 & 0.60 & 1.00 \\ 
  1.40 & 1.00 & 0.00 & 3.00 & 4.70 & 1.00 & 0.70 & 0.60 & 1.10 \\ 
  1.50 & 1.00 & 0.00 & 3.00 & 5.20 & 1.20 & 0.80 & 0.70 & 1.20 \\ 
  1.60 & 1.00 & 0.00 & 3.00 & 5.80 & 1.40 & 0.90 & 0.80 & 1.40 \\ 
  1.70 & 1.00 & 0.00 & 3.00 & 6.50 & 1.60 & 1.00 & 0.90 & 1.50 \\ 
  1.80 & 1.00 & 0.00 & 3.00 & 7.20 & 1.80 & 1.00 & 1.00 & 1.60 \\ 
  1.90 & 1.00 & 0.00 & 3.00 & 8.10 & 2.10 & 1.10 & 1.20 & 1.80 \\ 
  2.00 & 1.00 & 0.00 & 3.00 & 9.00 & 2.50 & 1.10 & 1.30 & 1.90 \\ 
  1.00 & 1.00 & 0.30 & 3.00 & 3.00 & 5.90 & 1.40 & 1.40 & 2.80 \\ 
  1.10 & 1.00 & 0.30 & 3.00 & 3.40 & 7.00 & 1.40 & 1.50 & 3.00 \\ 
  1.20 & 1.00 & 0.30 & 3.00 & 3.70 & 8.40 & 1.50 & 1.60 & 3.30 \\ 
  1.30 & 1.00 & 0.30 & 3.00 & 4.20 & 10.10 & 1.60 & 1.80 & 3.50 \\ 
  1.40 & 1.00 & 0.30 & 3.00 & 4.70 & 12.00 & 1.70 & 2.00 & 3.90 \\ 
  1.50 & 1.00 & 0.30 & 3.00 & 5.20 & 14.40 & 1.70 & 2.30 & 4.20 \\ 
  1.60 & 1.00 & 0.30 & 3.00 & 5.80 & 17.20 & 1.80 & 2.50 & 4.50 \\ 
  1.70 & 1.00 & 0.30 & 3.00 & 6.50 & 20.60 & 1.80 & 2.80 & 4.80 \\ 
  1.80 & 1.00 & 0.30 & 3.00 & 7.20 & 24.60 & 1.90 & 3.10 & 5.20 \\ 
  1.90 & 1.00 & 0.30 & 3.00 & 8.10 & 29.50 & 1.90 & 3.50 & 5.60 \\ 
  2.00 & 1.00 & 0.30 & 3.00 & 9.00 & 35.30 & 2.00 & 3.90 & 6.00 \\ 
  1.00 & 1.00 & 0.60 & 3.00 & 3.00 & 26.00 & 1.90 & 1.90 & 6.20 \\ 
  1.10 & 1.00 & 0.60 & 3.00 & 3.40 & 32.40 & 2.00 & 2.10 & 6.80 \\ 
  1.20 & 1.00 & 0.60 & 3.00 & 3.70 & 40.30 & 2.00 & 2.40 & 7.40 \\ 
  1.30 & 1.00 & 0.60 & 3.00 & 4.20 & 50.20 & 2.10 & 2.60 & 8.10 \\ 
  1.40 & 1.00 & 0.60 & 3.00 & 4.70 & 62.70 & 2.10 & 2.90 & 8.80 \\ 
  1.50 & 1.00 & 0.60 & 3.00 & 5.20 & 78.30 & 2.20 & 3.20 & 9.60 \\ 
  1.60 & 1.00 & 0.60 & 3.00 & 5.80 & 97.80 & 2.20 & 3.60 & 10.40 \\ 
  1.70 & 1.00 & 0.60 & 3.00 & 6.50 & 122.30 & 2.30 & 4.00 & 11.40 \\ 
  1.80 & 1.00 & 0.60 & 3.00 & 7.20 & 153.20 & 2.30 & 4.50 & 12.40 \\ 
  1.90 & 1.00 & 0.60 & 3.00 & 8.10 & 191.90 & 2.30 & 5.00 & 13.40 \\ 
  2.00 & 1.00 & 0.60 & 3.00 & 9.00 & 240.80 & 2.40 & 5.60 & 14.60 \\ 
   \hline
\end{tabular}
\endgroup
\end{table}


==> figures_tables/beta_qa_change_shape1_3_shape2_5_short.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Thu Feb 23 10:55:56 2023
\begin{table}[hp]
\centering
\caption{Design 4 with Beta(3,5)} 
\begingroup\footnotesize
\begin{tabular}{rrrrrrrrr}
  \hline
$q$ & $k$ & $a$ & $\bar{z}$ & $\bar{x}$ & $t_h$ & $z_h$ & $x_h$ & $s_h$ \\ 
  \hline
1.00 & 1.00 & 0.00 & 3.00 & 3.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.10 & 1.00 & 0.00 & 3.00 & 3.40 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.20 & 1.00 & 0.00 & 3.00 & 3.70 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.30 & 1.00 & 0.00 & 3.00 & 4.20 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.40 & 1.00 & 0.00 & 3.00 & 4.70 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.50 & 1.00 & 0.00 & 3.00 & 5.20 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.60 & 1.00 & 0.00 & 3.00 & 5.80 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.70 & 1.00 & 0.00 & 3.00 & 6.50 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.80 & 1.00 & 0.00 & 3.00 & 7.20 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.90 & 1.00 & 0.00 & 3.00 & 8.10 & 0.30 & 0.60 & 0.40 & 0.60 \\ 
  2.00 & 1.00 & 0.00 & 3.00 & 9.00 & 0.60 & 0.80 & 0.60 & 0.90 \\ 
  1.00 & 1.00 & 0.30 & 3.00 & 3.00 & 2.40 & 1.00 & 1.00 & 1.50 \\ 
  1.10 & 1.00 & 0.30 & 3.00 & 3.40 & 3.30 & 1.20 & 1.20 & 1.80 \\ 
  1.20 & 1.00 & 0.30 & 3.00 & 3.70 & 4.50 & 1.30 & 1.40 & 2.10 \\ 
  1.30 & 1.00 & 0.30 & 3.00 & 4.20 & 6.00 & 1.40 & 1.60 & 2.40 \\ 
  1.40 & 1.00 & 0.30 & 3.00 & 4.70 & 7.90 & 1.50 & 1.80 & 2.70 \\ 
  1.50 & 1.00 & 0.30 & 3.00 & 5.20 & 10.30 & 1.60 & 2.10 & 3.00 \\ 
  1.60 & 1.00 & 0.30 & 3.00 & 5.80 & 13.20 & 1.70 & 2.40 & 3.40 \\ 
  1.70 & 1.00 & 0.30 & 3.00 & 6.50 & 16.60 & 1.80 & 2.70 & 3.70 \\ 
  1.80 & 1.00 & 0.30 & 3.00 & 7.20 & 20.90 & 1.90 & 3.00 & 4.10 \\ 
  1.90 & 1.00 & 0.30 & 3.00 & 8.10 & 26.10 & 1.90 & 3.50 & 4.50 \\ 
  2.00 & 1.00 & 0.30 & 3.00 & 9.00 & 32.50 & 2.00 & 3.90 & 4.90 \\ 
  1.00 & 1.00 & 0.60 & 3.00 & 3.00 & 19.60 & 1.80 & 1.80 & 4.70 \\ 
  1.10 & 1.00 & 0.60 & 3.00 & 3.40 & 25.90 & 1.90 & 2.10 & 5.30 \\ 
  1.20 & 1.00 & 0.60 & 3.00 & 3.70 & 33.80 & 2.00 & 2.30 & 6.00 \\ 
  1.30 & 1.00 & 0.60 & 3.00 & 4.20 & 43.90 & 2.10 & 2.60 & 6.60 \\ 
  1.40 & 1.00 & 0.60 & 3.00 & 4.70 & 56.60 & 2.10 & 2.90 & 7.40 \\ 
  1.50 & 1.00 & 0.60 & 3.00 & 5.20 & 72.80 & 2.20 & 3.20 & 8.10 \\ 
  1.60 & 1.00 & 0.60 & 3.00 & 5.80 & 93.20 & 2.20 & 3.60 & 8.90 \\ 
  1.70 & 1.00 & 0.60 & 3.00 & 6.50 & 119.10 & 2.30 & 4.10 & 9.80 \\ 
  1.80 & 1.00 & 0.60 & 3.00 & 7.20 & 151.90 & 2.30 & 4.50 & 10.80 \\ 
  1.90 & 1.00 & 0.60 & 3.00 & 8.10 & 193.40 & 2.40 & 5.10 & 11.80 \\ 
  2.00 & 1.00 & 0.60 & 3.00 & 9.00 & 246.00 & 2.40 & 5.70 & 12.90 \\ 
   \hline
\end{tabular}
\endgroup
\end{table}


==> figures_tables/beta_qa_change_shape1_5_shape2_3_short.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Thu Feb 23 10:55:56 2023
\begin{table}[hp]
\centering
\caption{Design 4 with Beta(5,3)} 
\begingroup\footnotesize
\begin{tabular}{rrrrrrrrr}
  \hline
$q$ & $k$ & $a$ & $\bar{z}$ & $\bar{x}$ & $t_h$ & $z_h$ & $x_h$ & $s_h$ \\ 
  \hline
1.00 & 1.00 & 0.00 & 3.00 & 3.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.10 & 1.00 & 0.00 & 3.00 & 3.40 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.20 & 1.00 & 0.00 & 3.00 & 3.70 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.30 & 1.00 & 0.00 & 3.00 & 4.20 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.40 & 1.00 & 0.00 & 3.00 & 4.70 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.50 & 1.00 & 0.00 & 3.00 & 5.20 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.60 & 1.00 & 0.00 & 3.00 & 5.80 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.70 & 1.00 & 0.00 & 3.00 & 6.50 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.80 & 1.00 & 0.00 & 3.00 & 7.20 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.90 & 1.00 & 0.00 & 3.00 & 8.10 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2.00 & 1.00 & 0.00 & 3.00 & 9.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.00 & 1.00 & 0.30 & 3.00 & 3.00 & 2.40 & 0.90 & 0.90 & 1.60 \\ 
  1.10 & 1.00 & 0.30 & 3.00 & 3.40 & 2.70 & 0.90 & 0.90 & 1.80 \\ 
  1.20 & 1.00 & 0.30 & 3.00 & 3.70 & 3.20 & 1.00 & 1.00 & 1.90 \\ 
  1.30 & 1.00 & 0.30 & 3.00 & 4.20 & 3.80 & 1.10 & 1.10 & 2.10 \\ 
  1.40 & 1.00 & 0.30 & 3.00 & 4.70 & 4.60 & 1.20 & 1.30 & 2.30 \\ 
  1.50 & 1.00 & 0.30 & 3.00 & 5.20 & 5.60 & 1.30 & 1.40 & 2.60 \\ 
  1.60 & 1.00 & 0.30 & 3.00 & 5.80 & 7.00 & 1.40 & 1.60 & 2.90 \\ 
  1.70 & 1.00 & 0.30 & 3.00 & 6.50 & 8.90 & 1.50 & 1.90 & 3.20 \\ 
  1.80 & 1.00 & 0.30 & 3.00 & 7.20 & 11.40 & 1.50 & 2.20 & 3.50 \\ 
  1.90 & 1.00 & 0.30 & 3.00 & 8.10 & 14.60 & 1.60 & 2.50 & 3.90 \\ 
  2.00 & 1.00 & 0.30 & 3.00 & 9.00 & 18.70 & 1.70 & 2.90 & 4.30 \\ 
  1.00 & 1.00 & 0.60 & 3.00 & 3.00 & 13.50 & 1.60 & 1.60 & 4.30 \\ 
  1.10 & 1.00 & 0.60 & 3.00 & 3.40 & 17.90 & 1.70 & 1.80 & 4.90 \\ 
  1.20 & 1.00 & 0.60 & 3.00 & 3.70 & 23.80 & 1.80 & 2.00 & 5.50 \\ 
  1.30 & 1.00 & 0.60 & 3.00 & 4.20 & 31.60 & 1.90 & 2.30 & 6.20 \\ 
  1.40 & 1.00 & 0.60 & 3.00 & 4.70 & 41.60 & 2.00 & 2.60 & 6.90 \\ 
  1.50 & 1.00 & 0.60 & 3.00 & 5.20 & 54.70 & 2.00 & 2.90 & 7.70 \\ 
  1.60 & 1.00 & 0.60 & 3.00 & 5.80 & 71.40 & 2.10 & 3.30 & 8.60 \\ 
  1.70 & 1.00 & 0.60 & 3.00 & 6.50 & 93.00 & 2.20 & 3.70 & 9.50 \\ 
  1.80 & 1.00 & 0.60 & 3.00 & 7.20 & 120.50 & 2.20 & 4.20 & 10.40 \\ 
  1.90 & 1.00 & 0.60 & 3.00 & 8.10 & 155.70 & 2.30 & 4.70 & 11.50 \\ 
  2.00 & 1.00 & 0.60 & 3.00 & 9.00 & 200.60 & 2.30 & 5.30 & 12.60 \\ 
   \hline
\end{tabular}
\endgroup
\end{table}


==> figures_tables/beta_qa_change_shape1_5_shape2_5_short.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Thu Feb 23 10:55:56 2023
\begin{table}[hp]
\centering
\caption{Design 4 with Beta(5,5)} 
\begingroup\footnotesize
\begin{tabular}{rrrrrrrrr}
  \hline
$q$ & $k$ & $a$ & $\bar{z}$ & $\bar{x}$ & $t_h$ & $z_h$ & $x_h$ & $s_h$ \\ 
  \hline
1.00 & 1.00 & 0.00 & 3.00 & 3.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.10 & 1.00 & 0.00 & 3.00 & 3.40 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.20 & 1.00 & 0.00 & 3.00 & 3.70 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.30 & 1.00 & 0.00 & 3.00 & 4.20 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.40 & 1.00 & 0.00 & 3.00 & 4.70 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.50 & 1.00 & 0.00 & 3.00 & 5.20 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.60 & 1.00 & 0.00 & 3.00 & 5.80 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.70 & 1.00 & 0.00 & 3.00 & 6.50 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.80 & 1.00 & 0.00 & 3.00 & 7.20 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.90 & 1.00 & 0.00 & 3.00 & 8.10 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  2.00 & 1.00 & 0.00 & 3.00 & 9.00 & 0.00 & 0.00 & 0.00 & 0.00 \\ 
  1.00 & 1.00 & 0.30 & 3.00 & 3.00 & 1.50 & 0.80 & 0.80 & 1.20 \\ 
  1.10 & 1.00 & 0.30 & 3.00 & 3.40 & 1.80 & 0.80 & 0.80 & 1.30 \\ 
  1.20 & 1.00 & 0.30 & 3.00 & 3.70 & 2.20 & 0.90 & 0.90 & 1.50 \\ 
  1.30 & 1.00 & 0.30 & 3.00 & 4.20 & 2.90 & 1.00 & 1.10 & 1.70 \\ 
  1.40 & 1.00 & 0.30 & 3.00 & 4.70 & 3.80 & 1.20 & 1.20 & 2.00 \\ 
  1.50 & 1.00 & 0.30 & 3.00 & 5.20 & 5.20 & 1.30 & 1.50 & 2.30 \\ 
  1.60 & 1.00 & 0.30 & 3.00 & 5.80 & 7.20 & 1.40 & 1.80 & 2.60 \\ 
  1.70 & 1.00 & 0.30 & 3.00 & 6.50 & 9.90 & 1.50 & 2.10 & 3.00 \\ 
  1.80 & 1.00 & 0.30 & 3.00 & 7.20 & 13.20 & 1.60 & 2.40 & 3.40 \\ 
  1.90 & 1.00 & 0.30 & 3.00 & 8.10 & 17.50 & 1.70 & 2.80 & 3.90 \\ 
  2.00 & 1.00 & 0.30 & 3.00 & 9.00 & 22.70 & 1.80 & 3.30 & 4.30 \\ 
  1.00 & 1.00 & 0.60 & 3.00 & 3.00 & 13.60 & 1.60 & 1.60 & 4.10 \\ 
  1.10 & 1.00 & 0.60 & 3.00 & 3.40 & 18.90 & 1.80 & 1.90 & 4.70 \\ 
  1.20 & 1.00 & 0.60 & 3.00 & 3.70 & 25.80 & 1.90 & 2.10 & 5.40 \\ 
  1.30 & 1.00 & 0.60 & 3.00 & 4.20 & 34.70 & 2.00 & 2.40 & 6.10 \\ 
  1.40 & 1.00 & 0.60 & 3.00 & 4.70 & 46.10 & 2.00 & 2.70 & 6.80 \\ 
  1.50 & 1.00 & 0.60 & 3.00 & 5.20 & 60.70 & 2.10 & 3.00 & 7.60 \\ 
  1.60 & 1.00 & 0.60 & 3.00 & 5.80 & 79.30 & 2.20 & 3.40 & 8.40 \\ 
  1.70 & 1.00 & 0.60 & 3.00 & 6.50 & 103.10 & 2.20 & 3.90 & 9.30 \\ 
  1.80 & 1.00 & 0.60 & 3.00 & 7.20 & 133.40 & 2.30 & 4.30 & 10.30 \\ 
  1.90 & 1.00 & 0.60 & 3.00 & 8.10 & 171.90 & 2.30 & 4.90 & 11.30 \\ 
  2.00 & 1.00 & 0.60 & 3.00 & 9.00 & 220.90 & 2.30 & 5.50 & 12.50 \\ 
   \hline
\end{tabular}
\endgroup
\end{table}

